Digital Twin-based Out-of-Distribution Detection in Autonomous Vessels

An autonomous vessel (AV) is a complex cyber-physical system (CPS) with software enabling many key functionalities, e.g., navigation software enables an AV to autonomously or semi-autonomously follow a path to its destination. Digital twins of such AVs enable advanced functionalities such as running what-if scenarios, performing predictive maintenance, and enabling fault diagnosis. Due to technological improvements, real-time analyses using continuous data from vessels' real-time operations have become increasingly possible. However, the literature has little explored developing advanced analyses in real-time data in AVs with digital twins built with machine learning techniques. To this end, we present a novel digital twin-based approach (ODDIT) to detect future out-of-distribution (OOD) states of an AV before reaching them, enabling proactive intervention. Such states may indicate anomalies requiring attention (e.g., manual correction by the ship master) and assist testers in scenario-centered testing. The digital twin consists of two machine-learning models predicting future vessel states and whether the predicted state will be OOD. We evaluated ODDIT with five vessels across waypoint and zigzag maneuvering under simulated conditions, including sensor and actuator noise and environmental disturbances i.e., ocean current. ODDIT achieved high accuracy in detecting OOD states, with AUROC and TNR@TPR95 scores reaching 99\% across multiple vessels.

==> results/current_table.tex <==
% \begin{table}[h!]
% \centering
% \caption{OOD Detection Results for NPS AUV and Otter Vessels under Environmental Disturbances (i.e., ocean current)}
% \begin{tabular}{ccccccc}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{NPS AUV}}   & \multicolumn{3}{c}{\textbf{Otter}}    \\
% \cline{2-7}
%                         & Precision & Recall    & F1-Score  & Precision & Recall  & F1-Score \\
% \hline
% DTM-R                   & 0.4155    & 0.9967    & 0.5657    & 0.3472    & 1.0000  & 0.4616   \\
% DTM-E                   & 0.7569    & 0.8633    & 0.7739    & 0.5507    & 0.9467  & 0.6424   \\
% DTMC                    & \textbf{0.7974} & 0.9867 & \textbf{0.8737} & \textbf{0.7944} & 0.9967  & \textbf{0.8796} \\
% \hline
% \end{tabular}
% \end{table}


\begin{table}[h!]
\centering
\scriptsize
\caption{OOD Detection Results for NPS AUV, Otter, and Remus 100 Vessels under Environmental Disturbances (i.e., ocean current)}
\begin{tabular}{cccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{NPS AUV}} & \multicolumn{3}{c}{\textbf{Otter}} & \multicolumn{3}{c}{\textbf{Remus 100}} \\
\cline{2-10}
                        & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\
\hline
\textbf{DTM-R}                   & 0.4155 & 0.9967 & 0.5657 & 0.3472 & 1.0000 & 0.4616 & 0.0333 & 1.0000 & 0.0645 \\
\textbf{DTM-E}                   & 0.7569 & 0.8633 & 0.7739 & 0.5507 & 0.9467 & 0.6424 & 0.5091 & 0.9000 & 0.6405 \\
\textbf{DTMC}                    & 0.7974 & 0.9867 & 0.8737 & 0.7944 & 0.9967 & 0.8796 & 0.4859 & 0.9967 & 0.6470 \\
\hline
\end{tabular}
\end{table}


==> results/rq1-statistical-tests-auroc.tex <==
% \begin{table}[h!]
% \ra{1.2}
% \centering
% \caption{Dunn's Test \& Pairwise Comparisons - AUROC}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llccccccccl}
% \toprule
% Noise Magnitude & Vessel 1   & Vessel 2   & Comp. & \textit{p-value} & \vda{} & Magnitude \\
% \midrule
% m2  & Mariner & Remus 100   & Worse & < 0.05  & 0.18   & large \\
% \midrule
% m3  & Mariner & Remus 100   & Worse & < 0.05 & 0.03 & large \\
%      & Mariner & Otter   & Worse & < 0.05  & 0.08 & large \\
% \midrule
% m4  & Mariner & Remus 100   & Worse & < 0.05 & 0.03  & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05 & 0.07   & large \\
%      & Mariner & Otter   & Worse & < 0.05 & 0.04   & large \\
% \midrule
% m5  & Mariner & Remus 100   & Worse & < 0.05 & 0.04  & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05  & 0.09   & large \\
%      & Mariner & Otter   & Worse & < 0.05  & 0.08   & large \\
% \midrule
% m6  & Mariner & Remus 100   & Worse & < 0.05 & 0.06  & large \\
% \midrule
% m7  & Mariner & Remus 100   & Worse & < 0.05 & 0.01 & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05  & 0.02   & large \\
%      & Mariner & Otter   & Worse & < 0.05  & 0.01   & large \\
% \midrule
% m8  & Mariner & Remus 100   & Worse & < 0.05 & 0  & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05 & 0  & large \\
%      & Mariner & Otter   & Worse & < 0.05 & 0  & large \\
% \bottomrule
% \end{tabular}%
% }
% \label{tab:ship_comparison}
% \end{table}


% \begin{table}[h!]
% \ra{1.2}
% \centering
% \caption{Dunn's Test \& Pairwise Comparisons - TNR@TPR95}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llccccccccl}
% \toprule
% Noise Magnitude & Vessel 1   & Vessel 2   & Comp. & \textit{p-value} & \vda{} & Magnitude \\
% \midrule
% m2  & Mariner & Remus 100   & Worse & < 0.05  & 0.15   & large \\
% \midrule
% m3  & Mariner & Remus 100   & Worse & < 0.05 & 0.04 & large \\
%      & Mariner & Otter   & Worse & < 0.05  & 0.04 & large \\
% \midrule
% m4  & Mariner & Remus 100   & Worse & < 0.05 & 0.02  & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05 & 0.02   & large \\
%      & Mariner & Otter   & Worse & < 0.05 & 0.01   & large \\
% \midrule
% m5  & Mariner & Remus 100   & Worse & < 0.05 & 0.02  & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05  & 0.11   & large \\
% \midrule
% m6  & Mariner & Remus 100   & Worse & < 0.05 & 0.06  & large \\
%     & Mariner & NPS AUV  & Worse & < 0.05  & 0.08   & large \\
% \midrule
% m7  & Mariner & Remus 100   & Worse & < 0.05 & 0 & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05  & 0   & large \\
%      & Mariner & Otter   & Worse & < 0.05  & 0   & large \\
% \midrule
% m8  & Mariner & Remus 100   & Worse & < 0.05 & 0  & large \\
%      & Mariner & NPS AUV  & Worse & < 0.05 & 0  & large \\
%      & Mariner & Otter   & Worse & < 0.05 & 0  & large \\
% \bottomrule
% \end{tabular}%
% }
% \label{tab:ship_comparison}
% \end{table}


\begin{table}[h!]
\ra{1.2}
\centering
\caption{Dunn's Test \& Pairwise Comparisons - AUROC and TNR@TPR95}
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lllccccccc}
\toprule
\multirow{2}{*}{Noise Magnitude} & \multirow{2}{*}{Vessel 1} & \multirow{2}{*}{Vessel 2} & \multirow{2}{*}{Comp.} & \multirow{2}{*}{\textit{p-value}} & \multicolumn{2}{c}{AUROC} & \multicolumn{2}{c}{TNR@TPR95} \\
\cmidrule(lr){6-7} \cmidrule(lr){8-9}
& & & & & \vda{} & Magnitude & \vda{} & Magnitude \\
\midrule
m2  & Mariner & Remus 100   & Worse & < 0.05  & 0.18   & large & 0.15   & large \\
\midrule
m3  & Mariner & Remus 100   & Worse & < 0.05 & 0.03 & large & 0.04 & large \\
     & Mariner & Otter   & Worse & < 0.05  & 0.08 & large & 0.04 & large \\
\midrule
m4  & Mariner & Remus 100   & Worse & < 0.05 & 0.03  & large & 0.02  & large \\
     & Mariner & NPS AUV  & Worse & < 0.05 & 0.07   & large & 0.02   & large \\
     & Mariner & Otter   & Worse & < 0.05 & 0.04   & large & 0.01   & large \\
\midrule
m5  & Mariner & Remus 100   & Worse & < 0.05 & 0.04  & large & 0.02  & large \\
     & Mariner & NPS AUV  & Worse & < 0.05  & 0.09   & large & 0.11   & large \\
     & Mariner & Otter   & Worse & < 0.05  & 0.08   & large & -   & - \\
\midrule
m6  & Mariner & Remus 100   & Worse & < 0.05 & 0.06  & large & 0.06  & large \\
     & Mariner & NPS AUV  & Worse & < 0.05  & - & - & 0.08   & large \\
\midrule
m7  & Mariner & Remus 100   & Worse & < 0.05 & 0.01 & large & 0 & large \\
     & Mariner & NPS AUV  & Worse & < 0.05  & 0.02   & large & 0   & large \\
     & Mariner & Otter   & Worse & < 0.05  & 0.01   & large & 0   & large \\
\midrule
m8  & Mariner & Remus 100   & Worse & < 0.05 & 0  & large & 0  & large \\
     & Mariner & NPS AUV  & Worse & < 0.05 & 0  & large & 0  & large \\
     & Mariner & Otter   & Worse & < 0.05 & 0  & large & 0  & large \\
\bottomrule
\end{tabular}%
}
\label{tab:ship_comparison}
\end{table}



==> results/rq3_actuator_all_results.tex <==
\begin{table*}[h]
\centering
\caption{OOD detection results corresponding to extreme rudder angles with Spearman correlation coefficients}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll ccc ccl ccc ccl}
\toprule
& & \multicolumn{6}{c}{\textbf{AUROC}} & \multicolumn{6}{c}{\textbf{TNR@TPR95}} \\
\cmidrule(r){3-8} \cmidrule(l){9-14}
\textbf{Method} & \textbf{Vessel} & \textbf{ 40$^\circ$} & \textbf{45$^\circ$} & \textbf{50$^\circ$} & \textbf{Corr.} & \textbf{p-value} & \textbf{Strength} & \textbf{ 40$^\circ$} & \textbf{45$^\circ$} & \textbf{50$^\circ$} & \textbf{Corr.} & \textbf{p-value} & \textbf{Strength} \\
\midrule
\multirow{3}{*}{\approach{}} & Mariner & 97.92\% & 97.79\% & 94.67\% & 0.09 & > 0.05 & Very weak\textsuperscript{\(\neg\)} & 86.92\% & 95.28\% & 75.46\% & 0.27 & > 0.05 & Weak \\ 
& Container & 93.32\% & 91.88\% & 96.64\% & 0.27 & > 0.05 & Weak & 76.63\% & 74.60\% & 89.18\% & 0.33 & > 0.05 & Weak \\ 
& Remus 100 & 99.23\% & 98.56\% & 92.45\% & 0.65 & < 0.05\textsuperscript{\(\star\)} & Strong\textsuperscript{\(\neg\)} & 96.96\% & 94.82\% & 64.65\% & 0.58 & > 0.05 & Moderate\textsuperscript{\(\neg\)} \\ 
\midrule
\multirow{3}{*}{DTM-R} & Mariner & 92.89\% & 86.58\% & 89.31\% & 0.27 & > 0.05 & Weak\textsuperscript{\(\neg\)} & 55.57\% & 52.46\% & 28.91\% & 0.30 & > 0.05 & Weak\textsuperscript{\(\neg\)} \\ 
& Container & 89.70\% & 92.70\% & 91.42\% & 0.03 & > 0.05 & Very weak & 61.18\% & 69.29\% & 60.58\% & 0.12 & > 0.05 & Very weak\textsuperscript{\(\neg\)} \\ 
& Remus 100 & 95.80\% & 99.20\% & 99.23\% & 0.61 & < 0.05\textsuperscript{\(\star\)} & Strong & 80.85\% & 97.80\% & 98.84\% & 0.64 & < 0.05\textsuperscript{\(\star\)} & Strong \\ 
\midrule
\multirow{3}{*}{DTM-E} & Mariner & 44.30\% & 65.70\% & 72.35\% & 0.68 & < 0.05\textsuperscript{\(\star\)} & Strong & 5.08\% & 27.67\% & 34.11\% & 0.74 & < 0.05\textsuperscript{\(\star\)} & Strong \\ 
& Container & 66.99\% & 67.48\% & 66.29\% & -0.12 & > 0.05 & Very weak\textsuperscript{\(\neg\)} & 27.76\% & 21.48\% & 14.64\% & -0.03 & > 0.05 & Very weak\textsuperscript{\(\neg\)} \\ 
& Remus 100 & 90.11\% & 85.57\% & 72.97\% & -0.46 & > 0.05 & Moderate\textsuperscript{\(\neg\)} & 50.21\% & 49.55\% & 26.68\% & -0.25 & > 0.05 & Weak\textsuperscript{\(\neg\)} \\ 
\bottomrule
\end{tabular}%
}
\end{table*}


==> results/rq3_sensor_correlation_table.tex <==
\begin{table}[h]
    \centering
    \scriptsize
    % \renewcommand{\arraystretch}{1.2}
    \caption{Spearman correlation results for different OOD detection methods.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llccl ccl ccl}
        \toprule
        & & \multicolumn{3}{c}{\textbf{ODDIT}} & \multicolumn{3}{c}{\textbf{DTM-R}} & \multicolumn{3}{c}{\textbf{DTM-E}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        \textbf{Metric} & \textbf{Ship} & \textbf{Correlation} & \textbf{p-value} & \textbf{Strength} 
        & \textbf{Correlation} & \textbf{p-value} & \textbf{Strength} 
        & \textbf{Correlation} & \textbf{p-value} & \textbf{Strength} \\
        \midrule
        \multirow{4}{*}{AUROC} 
        & Mariner   & 0.02  & $>$ 0.05  & Very weak  & 0.27  & $<$ 0.05  & Weak  & 0.41  & $<$ 0.05  & Moderate \\
        & Remus 100 & 0.33  & $<$ 0.05  & Weak       & 0.61  & $<$ 0.05  & Strong & 0.42  & $<$ 0.05  & Moderate \\
        & NPS AUV   & 0.68  & $<$ 0.05  & Strong     & 0.53  & $<$ 0.05  & Moderate & 0.77  & $<$ 0.05  & Strong \\
        & Otter     & 0.61  & $<$ 0.05  & Strong     & 0.06 & $>$ 0.05  & Very weak\textsuperscript{\(\neg\)} & 0.64  & $<$ 0.05  & Strong \\
        \hline
        \multirow{4}{*}{TNR@TPR95} 
        & Mariner   & 0.01  & $>$ 0.05  & Very weak  & 0.31  & $<$ 0.05  & Weak  & 0.37  & $<$ 0.05  & Weak \\
        & Remus 100 & 0.32  & $<$ 0.05  & Weak       & 0.61  & $<$ 0.05  & Strong & 0.47  & $<$ 0.05  & Moderate \\
        & NPS AUV   & 0.70  & $<$ 0.05  & Strong     & 0.34  & $<$ 0.05  & Weak & 0.75  & $<$ 0.05  & Strong \\
        & Otter     & 0.60  & $<$ 0.05  & Strong     & 0.21 & $>$ 0.05  & Weak\textsuperscript{\(\neg\)} & 0.46  & $<$ 0.05  & Moderate \\
        \hline
    \end{tabular}%
    }
\end{table}

